F3B: A Low-Overhead Blockchain Architecture with Per-Transaction Front-Running Protection

Front-running attacks, which benefit from advanced knowledge of pending transactions, have proliferated in the blockchain space since the emergence of decentralized finance. Front-running causes devastating losses to honest participants and continues to endanger the fairness of the ecosystem. We present Flash Freezing Flash Boys (F3B), a blockchain architecture that addresses front-running attacks by using threshold cryptography. In F3B, a user generates a symmetric key to encrypt their transaction, and once the underlying consensus layer has finalized the transaction, a decentralized secret-management committee reveals this key. F3B mitigates front-running attacks because, before the consensus group finalizes it, an adversary can no longer read the content of a transaction, thus preventing the adversary from benefiting from advanced knowledge of pending transactions. Unlike other mitigation systems, F3B properly ensures that all unfinalized transactions, even with significant delays, remain private by adopting per-transaction protection. Furthermore, F3B addresses front-running at the execution layer; thus, our solution is agnostic to the underlying consensus algorithm and compatible with existing smart contracts. We evaluated F3B on Ethereum with a modified execution layer and found only a negligible (0.026%) increase in transaction latency, specifically due to running threshold decryption with a 128-member secret-management committee after a transaction is finalized; this indicates that F3B is both practical and low-cost.

==> Makefile <==
.PHONY: FORCE lenny all clean distclean pandoc

FILE=main

all: $(FILE).pdf

%.pdf: %.tex FORCE
	latexmk -pdf -f -e '$$pdflatex=q/pdflatex %O %S/' $<

fast:
	pdflatex $(FILE).tex && bibtex $(FILE).aux && pdflatex $(FILE).tex && pdflatex $(FILE).tex

clean:
	for ext in aux toc lof lot lol dlog bbl \
		tmp idv	lg 4tc 4ct xref	\
		nav snm fls vrb blg out tpt fdb_latexmk; \
	do \
		$(RM) $(FILE).$$ext ; \
	done
	$(RM) *.aux *.bak *~
	$(RM) *.log

distclean: clean
	$(RM) $(FILE).pdf
	$(RM) $(FILE).ps
	$(RM) $(FILE).dvi
	$(RM) $(FILE).css
	$(RM) *.html
	$(RM) *.docx
	$(RM) *.odt
	$(RM) *.d


==> content/layer.tex <==
\com{
\section{Mitigation at Different Layers}


\label{sec:layer}


From previous front-running mitigation work
~\cite{breidenbach2018enter,libsubmarine,ankalkoti2017relative,
kursawe2020wendy,kursawe2021wendy,saad2020frontrunning,ciampi2021fairmm},
we categorize those mitigation approaches into
two layers --- the blockchain layer and the application layer
%
Further, based on the layer that one chooses to address front-running,
we analyze the trade-offs inherently exhibited in their approaches.
We present an in-depth discussion of these trade-offs.
%
We consider the blockchain layer as the storage 
and consensus element of what makes a blockchain operable and
regard the application layer as the program element, such as
smart contracts agnostic to the underlying blockchain layer.
%

\begin{table*}[t]
\centering 
\caption{Comparison of front-running protection at different layers
\zhq{NOTE: This table is NOT intended to be in the AFT submission!
Reference Only!}}
\label{tab:comparsion} 
\begin{tabular}{l|c|c}
\toprule
 & Application Layer & Blockchain Layer  \\ 
                   \midrule
Definition of pending transaction & 
\makecell{Transactions that wait to be executed\\
 by a smart contract} &
\makecell{Transactions that wait to be committed \\
by the consensus group}  \\
\hline
Front-running attack vector & 
\makecell{Benefiting from pending transactions \\
in the application layer} &
\makecell{Benefiting from pending transactions \\
in the blockchain layer}  \\
\hline
Protection for scheduled AMM? & Yes & No \\
\hline
Protection scope & Specific smart contract & All smart contracts  \\
\hline
Modification of smart contract & Yes & Not Necessarily \\
\hline
Modification of blockchain & Not Necessarily & Yes \\
\hline
Compatibility & Various blockchains & Existing smart contracts \\
\hline
Smart contract address &
Hard to hide  &
Easy to hide \\
\hline
Examples&
Submarine~\cite{breidenbach2018enter, libsubmarine},
Namecoin~\cite{kalodner2015empirical},
FairMM~\cite{ciampi2021fairmm}&
Wendy~\cite{kursawe2020wendy,kursawe2021wendy}
CodeChain~\cite{saad2020frontrunning},
F3B \\
\bottomrule
\end{tabular} 
\end{table*}

Table \ref{tab:comparsion} demonstrates the key differences
between the mitigation strategies at two layers.
We now unpack the differences in detail.


\paragraph{Definition of Pending Transaction}
We define \emph{pending transactions} as transactions
that the relevant layer has not yet processed.
%
At the blockchain layer, this means that the transaction
is not committed---either sitting in mempool
or waiting for a certain number of block confirmations (for 
probabilistic consensus algorithms).
%
While at the application layer, this means
that the smart contract has not finalized the transaction.
%
A pending transaction can look differently in those two layers,
for example, when an explicit queue of transactions
is defined by a smart contract that are meant to be executed
sometime in the future: a prominent application that utilizes
these pending transaction queues is the scheduled 
AMMs~\cite{baum2021sok}.
%

\paragraph{Front-running Attack Vectors}
Given the different definitions for pending transactions,
there are two attack vectors: 
an attacker can launch front-running attacks
based on pending transactions
in application or blockchain layers.
Front-running attacks apply to both layers in most cases
but scheduled AMM might be different.
A scheduled AMM transaction may be committed in the blockchain, 
but its smart contract does not execute it due to the delayed execution;
thus, the attacker benefits from
a pending transaction in the application layer,
but not in the blockchain layer.


\paragraph{Mitigation Approaches:}
As each application is independent, 
the mitigation solution in the application layer
can only protect a specific smart contract
that adopts the solution,
while the solution in the blockchain layer
can protect all smart contracts at once.

\paragraph{Modification and Compatibility:}
The application layer’s mitigation solution
requires smart contract modification 
possibly without the need to fork the underlying blockchain
thus providing compatibility to various blockchains.
In some cases, as a solution requires additional functionality,
the blockchain needs a fork to provide the new function
~\cite{breidenbach2018enter, libsubmarine}.
On the other hand,
the mitigation solution in the blockchain layer
requires only a fork of the \ub,
possibly without the need to alter the smart contract,
thus providing compatibility with the existing smart contracts.

\paragraph{Side Channels:}
At the application
layer, an adversary can gain information about the smart contract
that a pending transaction invokes,
while at the blockchain layer,
an adversary is incapable of knowing which smart contract will be
executed, if the whole transaction is encrypted.
%
This knowledge gap is significant because even though an
approach can provide front-running protections, the adversary
can launch \emph{speculative} attacks using
the information at its disposal.
%
Items of information may include on-chain data such as 
the sender's balance for a given asset and 
the invoked smart contract~\cite{baum2021sok}.
%
Notably, front-running protection at the blockchain layer 
can easily ensure
that the invoked smart contract is hidden from public view 
by encrypting all transactions.
In contrast,
at the application layer, 
this protection is much harder and costly to deploy,
\eg, Submarine requires to send three transactions into the blockchain 
to hide the application's smart contract address
~\cite{breidenbach2018enter, libsubmarine}.
%
This information may unsuspectingly provide a significant advantage
to an adversary---in the case of an AMM with only two assets,
the adversary has at least a 50\% chance of choosing the right 
asset exchanging direction,
and by checking the sender's balance for these assets, 
this chance could increase to 100\%~\cite{baum2021sok}.
\\


%summary of F3B
\System's focus is on front-running protection at the blockchain
layer given the numerous benefits.
%
First, F3B has access to all transaction fields,
ensuring that F3B can hide fields that are not possible from the
application layer.
%
Second, all existing and new applications will immediately benefit 
from the front-running protection implemented at the blockchain
layer.
%
Recall that there are needs to be additional front-running protections that
may be necessary for certain applications such as scheduled AMMs.
%
Finally, any updates to the front-running protection is immediately
apply to all applications without their intervention.
%

\cb{The section presents a really nice comparison of tradeoffs in dealing with front running at application vs blockchain layer. I have one main question, due to two statements I see as conflicting. On the one hand, you said in the paragraph "front running attack vectors" that although a txn might already be committed in the blockchain, the smart contract may only execute it later. On the other hand, in later paragraphs you claim that countering front-running at the blockchain later also addresses front-running at the application layer. But, what if the application layer has a delayed execution, wouldn't front-running still be possible?}

\cb{I'd avoid the term "forking the blockchain", because most of the time forks have a negative implication and reviewers might think of unintentional forks. In my understanding, you're referring to scheduled forks caused by a change in blockchain implementation/algorithm. Thus, I'd change all appearances of "fork" in the paper to "scheduled fork".}
\veg{very good point about scheduled forks}

\cb{I agree that this section doesn't belong this early in the paper. I would, however, encourage you to have a discussion section; reviewers love discussion sections :), especially if you have more than one thing to discuss. One discussion topic would be in this case "App layer vs blockchain layer approaches". In the discussion, you could summarize some of the points in this section in 1-2 paragraphs, without the table. For example, I would add (1) the difference in meaning of comitting a txn in the blockchain vs application layer, and (2) the point on side channels, concluding with (3) that the blockchain approach is more general.}

\cb{Then, if the conference allows for it, I'd have an appendix that goes more in-depth in the topic and has the table. Also, the term "possibly no" in the table is confusing to me, consider replacing it with something else, for example "not necessarily".}

}

==> resources/latencyTable.tex <==
\begin{table}[t]
\centering 
\caption{Latency Overhead for Ethereum Blockchain}
\label{tab:latency} 
\begin{tabular}{cccccc}
\toprule
& \multicolumn{5}{c}{Latency Overhead for different size of SMC} \\ \cmidrule{2-6}
Confirmations & 8 & 16 & 32 & 64 & 128  \\ 
                   \midrule
5 & 0.05\%  & 0.10\%  & 0.24\%  & 0.74\%  & 2.73\%  \\ 
10 & 0.02\%  & 0.05\%  & 0.12\%  & 0.37\%  & 1.36\%  \\ 
20 & 0.01\%  & 0.03\%  & 0.06\%  & 0.19\%  & 0.68\%  \\ 
30 & 0.01\%  & 0.02\%  & 0.04\%  & 0.12\%  & 0.45\%  \\ 
50 & 0.00\%  & 0.01\%  & 0.02\%  & 0.07\%  & 0.27\%  \\ 
\bottomrule
\end{tabular} 
\end{table}


==> resources/latencyTableDela.tex <==
\begin{table}[t]
\centering 
\caption{Latency Overhead for Ethereum Blockchain}
\label{tab:latency} 
\begin{tabular}{cccccc}
\toprule
& \multicolumn{5}{c}{Latency Overhead for different size of SMC} \\ \cmidrule{2-6}
Confirmations & 8 & 16 & 32 & 64 & 128  \\ 
                   \midrule
0.02\%  & 0.02\%  & 0.02\%  & 0.03\%  & 0.05\%  \\ 
\bottomrule
\end{tabular} 
\end{table}



% \begin{table}[t]
% \centering 
% \caption{Latency Overhead for Ethereum Blockchain\zhq{We need to seperate them. You can ignore sizes for 8, 16 and 32, and put TDH2 and PVSS for 64 and 128.}}
% \label{tab:latency} 
% \begin{tabular}{cccccc}
% \toprule
% & \multicolumn{5}{c}{Latency Overhead for different size of SMC} \\ \cmidrule{2-6}
% Confirmations & 8 & 16 & 32 & 64 & 128  \\ 
%                    \midrule
% 8 & 0.135\%  & 0.159\%  & 0.167\%  & 0.249\%  & 0.297\%  \\ 
% 16 & 0.068\%  & 0.080\%  & 0.083\%  & 0.125\%  & 0.148\%  \\ 
% 32 & 0.034\%  & 0.040\%  & 0.042\%  & 0.062\%  & 0.074\%  \\ 
% 64 & 0.017\%  & 0.020\%  & 0.021\%  & 0.031\%  & 0.037\%  \\ 
% \bottomrule
% \end{tabular} 
% \end{table}

% \begin{table}[t]
% \centering 
% \caption{Latency Overhead for Ethereum Blockchain with PVSS}
% \label{tab:latency} 
% \begin{tabular}{cccccc}
% \toprule
% & \multicolumn{5}{c}{Latency Overhead for different size of SMC} \\ \cmidrule{2-6}
% Confirmations & 8 & 16 & 32 & 64 & 128  \\ 
%                    \midrule
% 8 & 0.140\%  & 0.150\%  & 0.188\%  & 0.250\%  & 0.331\%  \\ 
% 16 & 0.070\%  & 0.075\%  & 0.094\%  & 0.125\%  & 0.166\%  \\ 
% 32 & 0.035\%  & 0.038\%  & 0.047\%  & 0.063\%  & 0.083\%  \\ 
% 64 & 0.017\%  & 0.019\%  & 0.023\%  & 0.031\%  & 0.041\%  \\ 
% \bottomrule
% \end{tabular} 
% \end{table}

